Debugging Flaky Tests using Spectrum-based Fault Localization

Non-deterministically behaving (i.e., flaky) tests hamper regression testing as they destroy trust and waste computational and human resources. Eradicating flakiness in test suites is therefore an important goal, but automated debugging tools are needed to support developers when trying to understand the causes of flakiness. A popular example for an automated approach to support regular debugging is spectrum-based fault localization (SFL), a technique that identifies software components that are most likely the causes of failures. While it is possible to also apply SFL for locating likely sources of flakiness in code, unfortunately the flakiness makes SFL both imprecise and non-deterministic. In this paper we introduce SFFL (Spectrum-based Flaky Fault Localization), an extension of traditional coverage-based SFL that exploits our observation that 80% of flaky tests exhibit varying coverage behavior between different runs. By distinguishing between stable and flaky coverage, SFFL is able to locate the sources of flakiness more precisely and keeps the localization itself deterministic. An evaluation on 101 flaky tests taken from 48 open-source Python projects demonstrates that SFFL is effective: Of five prominent SFL formulas, DStar, Ochiai, and Op2 yield the best overall performance. On average, they are able to narrow down the fault's location to 3.5 % of the project's code base, which is 18.7 % better than traditional SFL (for DStar). SFFL's effectiveness, however, depends on the root causes of flakiness: The source of non-order-dependent flaky tests can be located far more precisely than order-dependent faults.

==> arxiv_submission/defs.tex <==

\usepackage[UKenglish]{babel}

\usepackage{booktabs}
\usepackage{url}
\def\UrlBreaks{\do\/\do-}

\usepackage{graphicx}
\graphicspath{{./images/}}
\usepackage{placeins}
\usepackage{subcaption}
\usepackage[justification=centering]{caption}
\usepackage{enumitem}
\usepackage{balance}
\usepackage{booktabs}  %
\usepackage{colortbl}

\usepackage{pgfplotstable}
\DeclareMathVersion{tabularbold}
\SetSymbolFont{operators}{tabularbold}{OT1}{cmr}{b}{n}

\usepackage{multirow}


\usepackage{inconsolata}

\usepackage{hyperref}

\usepackage[%
  group-minimum-digits=4,%
  list-final-separator={, and },%
  add-integer-zero=false,%
  free-standing-units,%
  binary-units,%
  detect-weight=true,%
  detect-inline-weight=math,%
]{siunitx}

\usepackage{microtype}

\usepackage[colorinlistoftodos,prependcaption,textsize=tiny
]{todonotes}

\newcommand{\gftodo}[1]{%
  \todo[color=green!40]{GF\@: #1}%
}
\newcommand{\gftodoil}[1]{%
  \todo[color=green!40,inline]{GF\@: #1}%
}
\newcommand{\mgtodoil}[1]{%
  \todo[color=blue!30,inline]{MG\@: #1}%
}
\newcommand{\mgtodo}[1]{%
  \todo[color=blue!30]{MG\@: #1}%
}
\newcommand{\pptodoil}[1]{%
  \todo[color=blue!30,inline]{PP\@: #1}%
}
\newcommand{\pptodo}[1]{%
  \todo[color=orange!30]{PP\@: #1}%
}
\newcommand{\done}[1]{%
  \todo[color=gray!40]{#1}%
}



\usepackage{xspace}

\usepackage[capitalise]{cleveref}

\crefformat{footnote}{#2\footnotemark[#1]#3}

\usepackage{tabularx}


\newcommand{\toolname}[1]{%
  \textsc{#1}\xspace%
}
\newcommand{\PyDefects}{%
  \toolname{PyDefects}%
}
\newcommand{\cmdtool}[1]{%
  \texttt{#1}\xspace%
}
\newcommand{\tabitem}{~~~}

\newcommand{\multilinecell}[1]{%
    \begin{tabular}{@{}r@{}}#1\end{tabular}
}
\newcommand{\multilinecellL}[1]{%
    \begin{tabular}{@{}l@{}}#1\end{tabular}
}
\newcommand{\multilinecellC}[1]{%
    \begin{tabular}{@{}c@{}}#1\end{tabular}
}
\newcommand{\multilinecellR}[1]{%
    \begin{tabular}{@{}r@{}}#1\end{tabular}
}

\newcommand{\summary}[2]{
    \vspace{0.6em}
    \noindent
    \colorbox{gray!20}{%
        \parbox{.97\linewidth}{%
                \textbf{Summary \textit{(#1)}}
            #2
        }%
    }%
}%

\usepackage{csquotes}
\usepackage{csvsimple}
\usepackage{listings}
\usepackage{xcolor}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{mystyle}{
  backgroundcolor=\color{backcolour},
  commentstyle=\color{codegreen},
  keywordstyle=\color{magenta},
  numberstyle=\tiny\color{codegray},
  stringstyle=\color{codepurple},
  basicstyle=\ttfamily\footnotesize,
  breakatwhitespace=false,
  breaklines=true,
  breakindent=60pt,
  captionpos=b,
  keepspaces=true,
  numbers=left,
  numbersep=5pt,
  showspaces=false,
  showstringspaces=false,
  showtabs=false,
  tabsize=2,
  numberblanklines=true,
  showlines=true,
  xleftmargin=2em,
  framexleftmargin=2.2em
}

\lstset{style=mystyle,language=Python,escapeinside=``}
\lstMakeShortInline[language=Python]|

\let\origthelstnumber\thelstnumber
\makeatletter
\newcommand*\Suppressnumber{%
  \lst@AddToHook{OnNewLine}{%
    \let\thelstnumber\relax%
     \advance\c@lstnumber-\@ne\relax%
    }%
}

\newcommand*\Reactivatenumber[1]{%
  \setcounter{lstnumber}{\numexpr#1-1\relax}
  \lst@AddToHook{OnNewLine}{%
   \let\thelstnumber\origthelstnumber%
   \refstepcounter{lstnumber}
  }%
}


